Unstructured Human Activity Detection from RGBD Images

Being able to detect and recognize human activities is essential for several applications, including personal assistive robotics. In this paper, we perform detection and recognition of unstructured human activity in unstructured environments. We use a RGBD sensor (Microsoft Kinect) as the input sensor, and compute a set of features based on human pose and motion, as well as based on image and pointcloud information. Our algorithm is based on a hierarchical maximum entropy Markov model (MEMM), which considers a person's activity as composed of a set of sub-activities. We infer the two-layered graph structure using a dynamic programming approach. We test our algorithm on detecting and recognizing twelve different activities performed by four people in different environments, such as a kitchen, a living room, an office, etc., and achieve good performance even when the person was not seen before in the training set.

==> algo_memm.tex <==

\iffalse

For the sake of understanding, we will first describe a single-layered MEMM model where
our goal is to predict the activity $y^t$ given the features $x^t$ at frame $t$.


\subsection{Single layered MEMM model}
% All human actions take time. We deal here with actions that typically take at least a few seconds, which means that an action will last for a few tens of frames. 

The structure of a one-layered MEMM model is shown in Figure \ref{fig:memm}.  It has the following terms:
\begin{itemize}
\item \textbf{$P(y^{(t)}|x^{(t)}$:}
This terms models the dependence of the activity label $y^t$ on the features $x^t$ computed
from the previous few frames. We can use several techniques to model this dependence.
In our full model (described in next section), we will use a Gaussian Mixture Model to model 
this term. We can use any classifier that also has a probabilistic interpretation. For comparison,
we also used multi-class support vector machines \cite{SVM-multiclass}. SVM is not intrinsically probabilistic, so we fit a sigmoid function to the multiclass SVM. The output of the sigmoid function gives us $P(y^{(t)}|x^{(t)})$. The parameters of the learning algorithm are learned from
the labeled training data.


\item \textbf{$y^{(t)}$ given $y^{(t-1)}$:}
Making an independent decision at every time step is not enough because activities
evolve over time. We can perform a better estimate of the activity at the current time,
if we also use the estimate of the activity at previous time-step.
For example, often the activities will last for a few tens of frames, therefore
the activity at time $t$ is likely to match the activity at time $(t-1)$. 
In addition, it is also likely that there are few frames of neutral activity between
two non-neutral activities, and some activities are more likely to follow others.
$P(y^{(t)}|y^{(t-1)})$ captures this intuition.

\end{itemize}

\noindent
\textbf{Inference.} 
Given the observation sequence up to time $t$, our goal is to can compute
$$
\alpha_t (j) = P(y^{(t)}=j|y^{(1)}, ..., y^{(t-1)}, x^{(1)}, ..., x^{(t)}),
$$
that is, the probability that the person is engaged in activity $j$ at time $t$. As shown by
\cite{Mccallum00maximumentropy}, this can be done with the Viterbi algorithm with a recursive Viterbi step
\begin{align*}
 \alpha_0 (j)&=P(y^{(t)}=j|x^{(t)}) \\
 \alpha_t (j)&=\sum_{k'\in Y}\alpha_{t-1}(k') \cdot P(y^{(t)}=j|y^{(t-1)}=k', x^{(t)})
\end{align*}

[[Perhaps need to shorten the rest of this inference section.]]

The probability of the current activity given the observation and previous activity,
$P(y^{t}|x^{t},y^{t-1})$, can be computed from probability values:
\begin{align*}
P(y^{t}|x^{t},y^{t-1})
&= {P(y^{t},x^{t}|y^{t-1}) \over P(x^{t}|y^{t-1})} \\
&= {P(y^{t-1}|y^t,x^t)P(y^t|x^t) \over P(y^{t-1}|x^t)}. \\
\intertext{By the naive Bayes conditional independence assumption, we assume that $y^{t-1}$ is independent of $x^t$ given $y^t$. Thus, the above formula becomes}
{P(y^{t-1}|y^t)P(y^t|x^t) \over P(y^{t-1}|x^t)}&= {P(y^t|y^{t-1})P(y^t|x^t) \over P(y^t)}
\end{align*}

The prior probability of each activity $P(y^{(t)})$ is given ahead of time and is often simply the uniform distribution. Thus, we already have all of the factors in the above formula, so we can compute $P(y^{t}|x^{t},y^{t-1})$, which then is used in computing $\alpha_t (j)$.


\fi


